Strangelets -- Effects of Finite Size and Exact Color Singletness

Matter consisting of up, down and strange quarks, socalled Strange Quark Matter, has been hypothesized to be stable in bulk, and conceivably stable or metastable in finite systems---strangelets---as an alternative state to ordinary baryonic matter. Strangelets, if they exist, may be relics from the hot and dense early universe, or they could be produced in high energy events, such as collisions of heavy nuclei at relativistic speeds. This thesis investigates the implications of various effects that affects the possible (meta-) stability of strangelets, such as finite size, distribution of quark states (shell model), interaction with a hadron gas, non-zero temperature and QCD constraints of color singletness of the wave function. These effects are studied within the phenomenological MIT bag model of quark matter using the multiple reflection expansion for a liquid drop model equation of state with comparison to a shell model. Finite size, non-zero temperature and color singlet constraints have a destabilizing effect on strangelets, and can suppress their production in heavy ion collisions. The work presented has been described in part in the following publications: Dan M{\o}nster Jensen and Jes Madsen, Strangelets at Non-Zero Temperature, in Strangeness and Quark Matter, edited by G. Vassiliadis, A. D. Panagiotou, S. Kumar, and J. Madsen (World Scientific, Singapore, 1995), pp. 220--229. Jes Madsen, Dan M. Jensen, and Michael B. Christiansen, Color Singlet Suppression of Quark-Gluon Plasma Formation, Phys. Rev. C 53, 1883 (1996). Dan M. Jensen and Jes Madsen, Strangelets with Finite Entropy, Phys. Rev. D 53, R4719 (1996). Dan M{\o}nster Jensen, Jes Madsen, and Michael B. Christiansen, Color Singlet Strangelets, Heavy Ion Phys. 4 (1-4), 387-394 (1996).

==> pressure.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\begin{picture}(1800,2069)(0,0)
\font\gnuplot=cmr10 at 10pt
\gnuplot
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(198.0,158.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(176,158){\makebox(0,0)[r]{-0.01}}
\put(1716.0,158.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(198.0,345.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(176,345){\makebox(0,0)[r]{-0.005}}
\put(1716.0,345.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(198.0,531.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(176,531){\makebox(0,0)[r]{0}}
\put(1716.0,531.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(198.0,718.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(176,718){\makebox(0,0)[r]{0.005}}
\put(1716.0,718.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(198.0,904.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(176,904){\makebox(0,0)[r]{0.01}}
\put(1716.0,904.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(198.0,1091.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(176,1091){\makebox(0,0)[r]{0.015}}
\put(1716.0,1091.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(198.0,1278.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(176,1278){\makebox(0,0)[r]{0.02}}
\put(1716.0,1278.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(198.0,1464.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(176,1464){\makebox(0,0)[r]{0.025}}
\put(1716.0,1464.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(198.0,1651.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(176,1651){\makebox(0,0)[r]{0.03}}
\put(1716.0,1651.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(198.0,1837.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(176,1837){\makebox(0,0)[r]{0.035}}
\put(1716.0,1837.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(198.0,2024.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(176,2024){\makebox(0,0)[r]{0.04}}
\put(1716.0,2024.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(198.0,158.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(198,113){\makebox(0,0){0}}
\put(198.0,2004.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(506.0,158.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(506,113){\makebox(0,0){0.2}}
\put(506.0,2004.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(813.0,158.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(813,113){\makebox(0,0){0.4}}
\put(813.0,2004.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1121.0,158.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1121,113){\makebox(0,0){0.6}}
\put(1121.0,2004.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1428.0,158.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1428,113){\makebox(0,0){0.8}}
\put(1428.0,2004.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1736.0,158.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1736,113){\makebox(0,0){1}}
\put(1736.0,2004.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(198.0,158.0){\rule[-0.200pt]{370.504pt}{0.400pt}}
\put(1736.0,158.0){\rule[-0.200pt]{0.400pt}{449.519pt}}
\put(198.0,2024.0){\rule[-0.200pt]{370.504pt}{0.400pt}}
\put(967,23){\makebox(0,0){$m /\mu$}}
\put(813,1278){\makebox(0,0)[l]{$p/\mu^4$}}
\put(275,531){\makebox(0,0)[l]{$\sigma /\mu^3$}}
\put(290,1651){\makebox(0,0)[l]{$\gamma /\mu^2$}}
\put(813,1278){\makebox(0,0)[l]{$p/\mu^4$}}
\put(275,531){\makebox(0,0)[l]{$\sigma /\mu^3$}}
\put(290,1651){\makebox(0,0)[l]{$\gamma /\mu^2$}}
\put(813,1278){\makebox(0,0)[l]{$p/\mu^4$}}
\put(275,531){\makebox(0,0)[l]{$\sigma /\mu^3$}}
\put(290,1651){\makebox(0,0)[l]{$\gamma /\mu^2$}}
\put(198.0,158.0){\rule[-0.200pt]{0.400pt}{449.519pt}}
\put(214,559){\usebox{\plotpoint}}
\multiput(214,559)(9.801,18.296){2}{\usebox{\plotpoint}}
\multiput(229,587)(10.878,17.677){2}{\usebox{\plotpoint}}
\put(255.66,630.77){\usebox{\plotpoint}}
\put(266.65,648.38){\usebox{\plotpoint}}
\multiput(276,663)(11.338,17.385){2}{\usebox{\plotpoint}}
\put(300.97,700.33){\usebox{\plotpoint}}
\put(312.74,717.42){\usebox{\plotpoint}}
\multiput(322,731)(12.579,16.510){2}{\usebox{\plotpoint}}
\put(349.66,767.55){\usebox{\plotpoint}}
\put(362.78,783.62){\usebox{\plotpoint}}
\put(376.11,799.53){\usebox{\plotpoint}}
\put(389.78,815.14){\usebox{\plotpoint}}
\put(403.99,830.26){\usebox{\plotpoint}}
\put(418.30,845.30){\usebox{\plotpoint}}
\put(433.10,859.84){\usebox{\plotpoint}}
\put(448.67,873.56){\usebox{\plotpoint}}
\put(463.96,887.59){\usebox{\plotpoint}}
\put(480.08,900.66){\usebox{\plotpoint}}
\put(496.47,913.38){\usebox{\plotpoint}}
\put(513.47,925.28){\usebox{\plotpoint}}
\put(530.53,937.08){\usebox{\plotpoint}}
\put(548.22,947.93){\usebox{\plotpoint}}
\put(566.50,957.75){\usebox{\plotpoint}}
\put(585.24,966.65){\usebox{\plotpoint}}
\put(604.33,974.78){\usebox{\plotpoint}}
\put(623.93,981.60){\usebox{\plotpoint}}
\put(643.74,987.68){\usebox{\plotpoint}}
\put(663.81,992.95){\usebox{\plotpoint}}
\put(684.25,996.57){\usebox{\plotpoint}}
\put(704.83,999.23){\usebox{\plotpoint}}
\put(725.51,1000.97){\usebox{\plotpoint}}
\put(746.26,1001.00){\usebox{\plotpoint}}
\put(767.02,1001.00){\usebox{\plotpoint}}
\put(787.64,999.05){\usebox{\plotpoint}}
\put(808.23,996.44){\usebox{\plotpoint}}
\put(828.72,993.18){\usebox{\plotpoint}}
\put(848.88,988.30){\usebox{\plotpoint}}
\put(869.02,983.25){\usebox{\plotpoint}}
\put(888.99,977.67){\usebox{\plotpoint}}
\put(908.53,970.68){\usebox{\plotpoint}}
\put(927.84,963.06){\usebox{\plotpoint}}
\put(947.17,955.52){\usebox{\plotpoint}}
\put(966.05,946.91){\usebox{\plotpoint}}
\put(984.96,938.35){\usebox{\plotpoint}}
\put(1003.59,929.21){\usebox{\plotpoint}}
\put(1021.92,919.48){\usebox{\plotpoint}}
\put(1039.96,909.22){\usebox{\plotpoint}}
\put(1057.86,898.71){\usebox{\plotpoint}}
\put(1075.95,888.53){\usebox{\plotpoint}}
\put(1093.58,877.61){\usebox{\plotpoint}}
\put(1111.08,866.45){\usebox{\plotpoint}}
\put(1128.42,855.05){\usebox{\plotpoint}}
\put(1145.99,844.01){\usebox{\plotpoint}}
\put(1163.24,832.46){\usebox{\plotpoint}}
\put(1180.38,820.75){\usebox{\plotpoint}}
\put(1197.59,809.16){\usebox{\plotpoint}}
\put(1214.55,797.20){\usebox{\plotpoint}}
\put(1231.47,785.18){\usebox{\plotpoint}}
\put(1248.37,773.13){\usebox{\plotpoint}}
\put(1265.35,761.20){\usebox{\plotpoint}}
\put(1282.18,749.06){\usebox{\plotpoint}}
\put(1299.23,737.22){\usebox{\plotpoint}}
\put(1316.33,725.46){\usebox{\plotpoint}}
\put(1333.11,713.24){\usebox{\plotpoint}}
\put(1350.23,701.51){\usebox{\plotpoint}}
\put(1367.46,689.94){\usebox{\plotpoint}}
\put(1384.61,678.26){\usebox{\plotpoint}}
\put(1401.81,666.63){\usebox{\plotpoint}}
\put(1419.00,655.00){\usebox{\plotpoint}}
\put(1436.48,643.82){\usebox{\plotpoint}}
\put(1454.23,633.06){\usebox{\plotpoint}}
\put(1472.28,622.81){\usebox{\plotpoint}}
\put(1489.74,611.63){\usebox{\plotpoint}}
\put(1508.17,602.09){\usebox{\plotpoint}}
\put(1526.35,592.08){\usebox{\plotpoint}}
\put(1545.07,583.16){\usebox{\plotpoint}}
\put(1563.93,574.50){\usebox{\plotpoint}}
\put(1582.96,566.22){\usebox{\plotpoint}}
\put(1602.28,558.64){\usebox{\plotpoint}}
\put(1621.85,551.72){\usebox{\plotpoint}}
\put(1641.63,545.43){\usebox{\plotpoint}}
\put(1661.73,540.30){\usebox{\plotpoint}}
\put(1682.11,536.38){\usebox{\plotpoint}}
\put(1702.62,533.30){\usebox{\plotpoint}}
\put(1723.32,531.79){\usebox{\plotpoint}}
\put(1736,531){\usebox{\plotpoint}}
\put(214,1947){\usebox{\plotpoint}}
\multiput(214,1947)(4.535,-20.254){4}{\usebox{\plotpoint}}
\multiput(229,1880)(4.890,-20.171){3}{\usebox{\plotpoint}}
\multiput(245,1814)(4.807,-20.191){3}{\usebox{\plotpoint}}
\multiput(260,1751)(5.186,-20.097){3}{\usebox{\plotpoint}}
\multiput(276,1689)(5.034,-20.136){3}{\usebox{\plotpoint}}
\multiput(291,1629)(5.519,-20.008){3}{\usebox{\plotpoint}}
\multiput(307,1571)(5.282,-20.072){3}{\usebox{\plotpoint}}
\multiput(322,1514)(5.702,-19.957){3}{\usebox{\plotpoint}}
\multiput(338,1458)(5.652,-19.971){2}{\usebox{\plotpoint}}
\multiput(353,1405)(5.998,-19.870){3}{\usebox{\plotpoint}}
\multiput(369,1352)(5.857,-19.912){3}{\usebox{\plotpoint}}
\multiput(384,1301)(6.443,-19.730){2}{\usebox{\plotpoint}}
\multiput(400,1252)(6.075,-19.846){3}{\usebox{\plotpoint}}
\multiput(415,1203)(6.689,-19.648){2}{\usebox{\plotpoint}}
\multiput(431,1156)(6.953,-19.556){2}{\usebox{\plotpoint}}
\multiput(447,1111)(6.697,-19.645){3}{\usebox{\plotpoint}}
\multiput(462,1067)(7.238,-19.453){2}{\usebox{\plotpoint}}
\multiput(478,1024)(6.981,-19.546){2}{\usebox{\plotpoint}}
\multiput(493,982)(7.546,-19.335){2}{\usebox{\plotpoint}}
\multiput(509,941)(7.451,-19.372){2}{\usebox{\plotpoint}}
\multiput(524,902)(8.054,-19.129){2}{\usebox{\plotpoint}}
\multiput(540,864)(7.798,-19.235){2}{\usebox{\plotpoint}}
\multiput(555,827)(8.629,-18.877){2}{\usebox{\plotpoint}}
\multiput(571,792)(8.176,-19.077){2}{\usebox{\plotpoint}}
\put(593.52,741.48){\usebox{\plotpoint}}
\multiput(602,724)(8.809,-18.793){2}{\usebox{\plotpoint}}
\multiput(617,692)(9.519,-18.444){2}{\usebox{\plotpoint}}
\put(639.65,648.54){\usebox{\plotpoint}}
\multiput(649,631)(9.536,-18.435){2}{\usebox{\plotpoint}}
\multiput(664,602)(10.298,-18.021){2}{\usebox{\plotpoint}}
\put(689.23,557.39){\usebox{\plotpoint}}
\multiput(695,547)(11.188,-17.482){2}{\usebox{\plotpoint}}
\put(721.65,504.25){\usebox{\plotpoint}}
\put(733.02,486.90){\usebox{\plotpoint}}
\multiput(742,474)(11.338,-17.385){2}{\usebox{\plotpoint}}
\put(768.57,435.82){\usebox{\plotpoint}}
\put(780.81,419.06){\usebox{\plotpoint}}
\put(793.41,402.58){\usebox{\plotpoint}}
\put(806.67,386.62){\usebox{\plotpoint}}
\multiput(819,371)(14.225,-15.114){2}{\usebox{\plotpoint}}
\put(847.59,339.74){\usebox{\plotpoint}}
\put(862.48,325.30){\usebox{\plotpoint}}
\put(877.62,311.11){\usebox{\plotpoint}}
\put(892.79,296.93){\usebox{\plotpoint}}
\put(908.63,283.55){\usebox{\plotpoint}}
\put(924.81,270.55){\usebox{\plotpoint}}
\put(941.74,258.55){\usebox{\plotpoint}}
\put(958.99,247.01){\usebox{\plotpoint}}
\put(977.10,236.88){\usebox{\plotpoint}}
\put(995.49,227.25){\usebox{\plotpoint}}
\put(1014.36,218.65){\usebox{\plotpoint}}
\put(1033.74,211.22){\usebox{\plotpoint}}
\put(1053.40,204.56){\usebox{\plotpoint}}
\put(1073.36,198.99){\usebox{\plotpoint}}
\put(1093.74,195.05){\usebox{\plotpoint}}
\put(1114.27,192.09){\usebox{\plotpoint}}
\put(1134.99,191.00){\usebox{\plotpoint}}
\put(1155.74,191.00){\usebox{\plotpoint}}
\put(1176.38,192.92){\usebox{\plotpoint}}
\put(1197.01,194.94){\usebox{\plotpoint}}
\put(1217.39,198.88){\usebox{\plotpoint}}
\put(1237.58,203.65){\usebox{\plotpoint}}
\put(1257.53,209.32){\usebox{\plotpoint}}
\put(1277.06,216.35){\usebox{\plotpoint}}
\put(1296.35,223.96){\usebox{\plotpoint}}
\put(1315.36,232.28){\usebox{\plotpoint}}
\put(1334.16,241.08){\usebox{\plotpoint}}
\put(1352.53,250.72){\usebox{\plotpoint}}
\put(1370.45,261.19){\usebox{\plotpoint}}
\put(1388.10,272.07){\usebox{\plotpoint}}
\put(1405.59,283.24){\usebox{\plotpoint}}
\put(1422.54,295.20){\usebox{\plotpoint}}
\put(1439.59,307.03){\usebox{\plotpoint}}
\put(1456.36,319.27){\usebox{\plotpoint}}
\put(1472.94,331.75){\usebox{\plotpoint}}
\put(1489.20,344.65){\usebox{\plotpoint}}
\put(1505.72,357.21){\usebox{\plotpoint}}
\put(1521.75,370.39){\usebox{\plotpoint}}
\put(1537.53,383.87){\usebox{\plotpoint}}
\put(1553.55,397.07){\usebox{\plotpoint}}
\put(1569.34,410.53){\usebox{\plotpoint}}
\put(1585.34,423.76){\usebox{\plotpoint}}
\put(1601.00,437.37){\usebox{\plotpoint}}
\put(1616.64,451.02){\usebox{\plotpoint}}
\put(1632.47,464.44){\usebox{\plotpoint}}
\put(1648.61,477.49){\usebox{\plotpoint}}
\put(1664.98,490.24){\usebox{\plotpoint}}
\put(1681.65,502.61){\usebox{\plotpoint}}
\put(1698.87,514.17){\usebox{\plotpoint}}
\put(1716.94,524.37){\usebox{\plotpoint}}
\put(1736,531){\usebox{\plotpoint}}
\put(214,1476){\usebox{\plotpoint}}
\put(214.00,1476.00){\usebox{\plotpoint}}
\put(234.71,1474.64){\usebox{\plotpoint}}
\put(255.35,1472.62){\usebox{\plotpoint}}
\put(275.79,1469.04){\usebox{\plotpoint}}
\put(296.09,1464.73){\usebox{\plotpoint}}
\put(316.19,1459.55){\usebox{\plotpoint}}
\put(336.07,1453.60){\usebox{\plotpoint}}
\put(355.74,1446.97){\usebox{\plotpoint}}
\put(375.12,1439.55){\usebox{\plotpoint}}
\put(394.25,1431.51){\usebox{\plotpoint}}
\put(413.12,1422.88){\usebox{\plotpoint}}
\put(431.71,1413.64){\usebox{\plotpoint}}
\put(450.14,1404.11){\usebox{\plotpoint}}
\put(468.04,1393.60){\usebox{\plotpoint}}
\put(485.76,1382.83){\usebox{\plotpoint}}
\put(503.22,1371.61){\usebox{\plotpoint}}
\put(520.60,1360.27){\usebox{\plotpoint}}
\put(537.73,1348.56){\usebox{\plotpoint}}
\put(554.06,1335.75){\usebox{\plotpoint}}
\put(571.11,1323.91){\usebox{\plotpoint}}
\put(587.35,1310.99){\usebox{\plotpoint}}
\put(603.84,1298.40){\usebox{\plotpoint}}
\put(619.60,1284.89){\usebox{\plotpoint}}
\put(635.70,1271.80){\usebox{\plotpoint}}
\put(651.74,1258.63){\usebox{\plotpoint}}
\put(667.41,1245.02){\usebox{\plotpoint}}
\put(682.94,1231.25){\usebox{\plotpoint}}
\put(698.21,1217.19){\usebox{\plotpoint}}
\put(713.66,1203.34){\usebox{\plotpoint}}
\put(728.48,1188.83){\usebox{\plotpoint}}
\put(743.98,1175.02){\usebox{\plotpoint}}
\put(758.71,1160.40){\usebox{\plotpoint}}
\put(773.82,1146.18){\usebox{\plotpoint}}
\multiput(788,1132)(15.142,-14.196){2}{\usebox{\plotpoint}}
\put(818.34,1102.66){\usebox{\plotpoint}}
\put(833.02,1087.98){\usebox{\plotpoint}}
\put(847.69,1073.31){\usebox{\plotpoint}}
\put(862.76,1059.03){\usebox{\plotpoint}}
\put(877.54,1044.46){\usebox{\plotpoint}}
\put(892.22,1029.78){\usebox{\plotpoint}}
\put(906.89,1015.11){\usebox{\plotpoint}}
\put(921.57,1000.43){\usebox{\plotpoint}}
\put(936.24,985.76){\usebox{\plotpoint}}
\put(950.92,971.08){\usebox{\plotpoint}}
\put(965.60,956.40){\usebox{\plotpoint}}
\put(980.27,941.73){\usebox{\plotpoint}}
\put(995.11,927.21){\usebox{\plotpoint}}
\put(1010.12,912.88){\usebox{\plotpoint}}
\put(1024.92,898.33){\usebox{\plotpoint}}
\put(1039.96,884.04){\usebox{\plotpoint}}
\put(1054.72,869.45){\usebox{\plotpoint}}
\put(1069.92,855.32){\usebox{\plotpoint}}
\put(1085.45,841.55){\usebox{\plotpoint}}
\put(1100.20,826.95){\usebox{\plotpoint}}
\put(1115.80,813.26){\usebox{\plotpoint}}
\put(1131.03,799.16){\usebox{\plotpoint}}
\put(1147.07,786.00){\usebox{\plotpoint}}
\put(1162.32,771.93){\usebox{\plotpoint}}
\put(1178.39,758.79){\usebox{\plotpoint}}
\put(1194.20,745.35){\usebox{\plotpoint}}
\put(1210.65,732.70){\usebox{\plotpoint}}
\put(1226.64,719.50){\usebox{\plotpoint}}
\put(1243.49,707.41){\usebox{\plotpoint}}
\put(1260.01,694.87){\usebox{\plotpoint}}
\put(1276.96,682.89){\usebox{\plotpoint}}
\put(1293.89,670.89){\usebox{\plotpoint}}
\put(1311.29,659.57){\usebox{\plotpoint}}
\put(1328.66,648.22){\usebox{\plotpoint}}
\put(1346.20,637.13){\usebox{\plotpoint}}
\put(1364.02,626.49){\usebox{\plotpoint}}
\put(1382.44,616.94){\usebox{\plotpoint}}
\put(1400.50,606.75){\usebox{\plotpoint}}
\put(1419.18,597.71){\usebox{\plotpoint}}
\put(1438.14,589.25){\usebox{\plotpoint}}
\put(1457.01,580.62){\usebox{\plotpoint}}
\put(1476.40,573.24){\usebox{\plotpoint}}
\put(1495.92,566.21){\usebox{\plotpoint}}
\put(1515.73,560.02){\usebox{\plotpoint}}
\put(1535.75,554.56){\usebox{\plotpoint}}
\put(1555.86,549.44){\usebox{\plotpoint}}
\put(1576.11,544.92){\usebox{\plotpoint}}
\put(1596.48,540.94){\usebox{\plotpoint}}
\put(1617.06,538.32){\usebox{\plotpoint}}
\put(1637.65,535.67){\usebox{\plotpoint}}
\put(1658.33,533.98){\usebox{\plotpoint}}
\put(1679.04,532.66){\usebox{\plotpoint}}
\put(1699.76,531.33){\usebox{\plotpoint}}
\put(1720.50,531.00){\usebox{\plotpoint}}
\put(1736,531){\usebox{\plotpoint}}
\end{picture}

